Enforcing safety for vision-based controllers via Control Barrier Functions and Neural Radiance Fields

To navigate complex environments, robots must increasingly use high-dimensional visual feedback (e.g. images) for control. However, relying on high-dimensional image data to make control decisions raises important questions; particularly, how might we prove the safety of a visual-feedback controller? Control barrier functions (CBFs) are powerful tools for certifying the safety of feedback controllers in the state-feedback setting, but CBFs have traditionally been poorly-suited to visual feedback control due to the need to predict future observations in order to evaluate the barrier function. In this work, we solve this issue by leveraging recent advances in neural radiance fields (NeRFs), which learn implicit representations of 3D scenes and can render images from previously-unseen camera perspectives, to provide single-step visual foresight for a CBF-based controller. This novel combination is able to filter out unsafe actions and intervene to preserve safety. We demonstrate the effect of our controller in real-time simulation experiments where it successfully prevents the robot from taking dangerous actions.

==> response.tex <==
\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{subcaption}
\usepackage{mymacros}
\usepackage{comment}
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\usepackage{geometry}

Comments to author (Associate Editor) ===================================== This paper focuses on visual-based control, and proposes an approach that combines discrete-time control barrier functions (CBFs) with neural radiance fields (NeRFs) for prediction-based safe control of a mobile robot. The work is validated in simulation on two robots in the same environment. First of all, all reviewers agree that this work is highly relevant to the field, and proposes an interesting contributions. The paper is well written and pleasant to read. However, a few reviewers mention that some of the key concepts should be better introduced, as the work currently seems to be written for an audience familiar with CBFs and NeRFs, which seems like a strong requirement. A few inaccurate statements also need to be corrected, and a few references added and discussed. More importantly, the results need to be expanded, to consider more than just a single environment and two robots. ---------------------------------------- Comments on Video Attachment: All reviewers agree that the video is helpful and a good companion to the paper. Comments to author (Editor) ================================ See the AE report for an overview and the individual reviews for specific suggestions regarding how the paper could be improved. ---------------------------------------- Comments on Video Attachment: Satisfactory

2693
I would like to thank the authors for their submission. They present an interesting work combining two popular methods, one in control and another in computer vision. Their main contributions are: 1. a CBF which relies solely on high-dimensional visual (RGBD) NeRF estimates, 2. a controller which relies on NeRF hallucinations to provide the single-step look-ahead 3. a demonstration the capabilities of this contoller in real-time simulation. Major Comments: 

- The paper focuses on a discrete-time application of CBFs which requires an ability to predict future observations in order to evaluate the barrier function. To a reader who is unfamiliar with CBFs this is confusing since the continuous-time CBF [3] is more common and does not require this one-step look-ahead ability. Clarity would be improved if the discrete-time nature were emphasized throughout the paper including the abstract, discussion of (1), and perhaps the title. 

\textbf{We have stressed the disrecte-time nature of our CBF in the revised paper.}

- The manuscript cites [11] as a paper which utilizes a bounded-error state-estimation oracle in conjunction with CBFs however it appears that this paper uses a system-level synthesis (SLS) method instead of a CBF one to achieve robustness. [11] is again mentioned in Section VI saying that it contains error-robust CBFs, but it does not. 

\textbf{We have replaced it with the correct paper.}

- The authors make claims about the difference between NeRF-based density and depth estimates and argue that their use of depth is better than NeRF-NAVIGATION's use of density. However, the mathematical distinction between the NeRF depth and density is unexplained. How are the density and the depth related? The paper would benefit greatly from a mathematical description of the relationship between these two quantities. For example, in the experiments, what do the density values of {-40, -30, -20} indicate? 

\textbf{The NeRF density refers the differential probability of a spatial point terminating a ray of light. The probability of stopping light is assumed as a strong proxy for the probability of terminating a mass particle. Thus, the collision probability at time t is given by}

\added{\begin{subequations}
\begin{align}
p_t^{coll}=P(\bigcup_{\mathbf{b_t}\in\mathcal{B}}\mathbf{b_t}\in\mathcal{X}_{coll}) \geq{\sum_{\mathbf{b_t}\in\mathcal{B}}}\rho(\mathbf{b_t})s(\mathbf{b_t})
\end{align}
\end{subequations}}

\textbf{where $\mathcal{X}_{coll}$ denotes the collision set, $s(\mathbf{b_t})$ is the distance traveled by a body-fixed point $\mathbf{b}$ in timestep $\mathbf{t}$, and the bound follows from Boole’s inequality. Therefore, density values must be non-negative. The depth of a point in the image is the distance between the camera and that point, where a ray of light to this direction emitted from the camera stops. Depth is normally calculated by integrating the density field along rays.}

- It should be noted that this work and NeRF-NAVIGATION have different goals. Yes this work succeeds in achieving faster execution time, but it does so while accomplishing a subset of NeRF-NAVIGATIONS goals. This work attempts to keep the system safe using the NeRF whereas NeRF-NAVIGATION appears to keep the system safe while also navigating to the goal state. If this is correct, the difference between the alogrithms' goals should be mentioned. 

\textbf{Although our work and NeRF-NAVIGATION have different goals (safety filter vs trajectory planning), NeRF-NAVIGATION is the only work we're aware of doing planning based on NeRFs and so we compare with it anyway. We have clarified this in the revised paper.}

- Although it is true that the authors succeed in running in real time, the computer and graphics processor used are much more powerful than those common on robotics platforms, including those optimized for vision-based control [see "Agilicious: Open-source and open-hardware agile quadrotor for vision-based flight", P Foehn, et al. Science Robotics, 2022]. An evaluation of this method on a more common embedded computer such as an Nvidia Jetson TX2 or Xavier would elevate the applicability of this work since most robots would be unable to carry and power a 3090 GPU. 

\textbf{In the future work we can run in real time on desktop hardware, and an area of future work involves reducing the computational needs of the NeRF to run in real time on embedded hardware. We have added the relative discussion to the paper.}

- This work claims to be the first to use direct visual-feedback for the CBF. Although they do not use NeRFs, it appears that "Self-Supervised Online Learning for Safety-Critical Control using Stereo Vision" [Cosner, et al. ICRA, 2022] may have achieved a similar feat by operating on the pixel-wise disparity observed on stereo-images. 

\textbf{Sure. We have changed our statement in II-B to ‘CBFs have not previously seen much use in the direct visual-feedback setting’.}

--- Minor Comments: - Charles Dawson and Chuchu Fan are listed as having the same email address. 

\textbf{We have changed it.}

- You note that you can deal with field-of-view problems by adding additional cameras, however this would significantly impact rendering speeds, correct? Since you would need to render significantly more pixels per action. 

\textbf{Sure. We need to consider ensuring that the system can run in real time. Probably reducing the camera/nerf resolution could help with rendering time. We have added the relative discussion to the paper.}

- It is clear that the NeRF provides a method by which to hallucinate possible future depth estimates, but would it be possible (and perhaps much faster) to estimate the future depth using the dynamics model? Perhaps, in future work, the two methods could be used in conjunction for filtering. 

\textbf{We do not know any method that can achieve this goal, but we can set this as one direction of our future work since the acceleration of computation is an essential point that we need to consider.}

- The introduction could benefit from a discussion about imitation learning-based pixel controllers such as the one presented in "Agile Autonomous Driving using End-to-End Deep Imitation Learning" [Pan et al 2017]. These type of controllers have been a popular way of combining control and vision, but lack the safety guarantees that are presented in the here. This work represents an important step forward from those works. 

\textbf{We have added it to the paper.}

- I would consider writing out the acronym Simultaneous Localization And Mapping (SLAM) when it is first introduced. 

\textbf{We have added it to the paper.}

- the authors mention that they use a two-level control architecture where the high-level CBF controller utilizes a simple dynamics model and the low-level tracks that desired trajectory. What are the low-level dynamics and controllers for the simulation? Or are the low-level complexities ignored for this work? 

\textbf{The low-level complexities ignored for this work, but we can build a model for the low-level issues in future work.}

- In Section IV C there is a minor typo: "This capability allows us the robot [...]" 

\textbf{We have deleted ‘us’.}

- The size of the text in Figure 1 is difficult to read due to its size.

\textbf{We have enlarged the size of the text.}

2695
Paper summery: - The paper combines the techniques from Neural Radiance Fields and Control Barrier Functions to make a controller to that prevents a robot from executing unsafe actions - It uses the NeRF to predict what a future state might look like, this is used as input to a CBF that determines and avoids unsafe actions - It shows the method working on several simplified robot models in simulation Paper Clarity: - Overall the paper is very clear in describing the method and giving background on the underlying methods. 

- What are the transparent shaded areas in Figure 3? They looks like standard deviation over multiple runs but I don't think this is explained anywhere. 

\textbf{Yes, they are standard deviations over multiple runs. We have added this note to the paper.} 

Recommendations: - The paper does lack in the experimental section. It only uses one environment and only two very simple robot dynamics I would like to see results with a system more complex than a single or double integrator. Ideally in more then one environment. I think a good addition would be a 2D planar robot shown to be avoiding collision with an obstacle in a room. 

\textbf{Deploying these methods on a ground robot is an important next step for our future work, and we will also conduct experiments on more environments later.}

- The CBF interferes only in the last time step. I would be interested to see how it fairs for example in the double integrator system with higher velocities/lower max accelerations. 

\textbf{CBF does not only interfere in the last few time steps. As can been seen in Figure 3 and Figure 4, CBF judges the intended actions as dangerous around 2s, since action interventions (the red curves) rised up over 0. No matter how high the velocities or how low the max accelerations, the rationale of our controller indicates that it will act when the intended action can induce collision with obstacles.}

- The ablation study shows a CBF on the NeRF rendered images outperforming a CBF directly based on the NeRF density. Whats interesting is the image based CBF takes the minimum distance over the image frame while the direct NeRF density CBF samples only one point. I wonder if the performance difference would still be there if you took multiple random samples around the x position and used the max density. 

\textbf{As in some occasions the density map can be roughly constructed, which might cause danger like collision (as shown in contrast experiments for NeRF-Navigation), this is an instinct potential drawback of using density maps to judge the safety of the system. In this way, almost all the methods based on density maps can lead to failure including collision. However, our method directly utilizes the observed depth data to ensure the security, so it can avoid this flaw at ease.}

- The paper does feel a bit simplistic. The CBF is a hand coded function/heuristic, so it feels like the magic is in hand crafting a CBF for a given situation that keeps the robot safe. The issue is that while writing one for a simple system is easy, writing one for a more realistic system is non trivial. That being said: using NeRF for controls is a very new field and to my knowledge combining NeRFs and CBFs is both novel and important.

\textbf{We just utilize simple hand-made CBFs to ensure the speed of computation, i.e. we try to strike a balance between the effect of control and the operation efficiency. We can think of more complicated forms of CBF in the future to better simulate the realistic environments where there are unignorable noises.}

The accompanying video is helpful in showing intermediate frames of the experiment. What I think would be helpful is an external view or plot showing the position of the robot.

2697
In this paper, control barrier functions with visual feedback are used to enforce safety for vision-based controllers. Neural radiance fields are used to learn implicit representations of 3D scenes and predict future observations in order to evaluate the barrier function. Simulation studies show the viability of the proposed approach. The paper is well-organized and easy to read. The reviewer has the following comments. 

1. The 'Minimal intervention' is listed as a requirement in the problem statement and also in equation (1a). However, I do not think the authors solved this problem. More discussions are needed to justify (1a) and the 'Minimal intervention' are satisfied with the proposed approach. This may be a disadvantage compared to CBFs with state feedback. 

\textbf{In this work we in fact do not exactly achieve the goal of minimal intervention, since we just randomly resample a batch of actions around the intended action and select the one that is the closest to the input. We can explore more efficient methods to make the controller gratify this requirement.}

2. The advantage of the proposed approach compared with methods with regular CBFs and state estimation is not clear. CBFs have been used to deal with moving obstacles. There may be a problem with the statement 'Previous works have shown that CBFs defined as functions of state do not generalize well to new environments (e.g. when obstacles have moved)'. Also, related works such as Measurement-Robust Control Barrier Functions may be discussed.

\textbf{Our paper is meant as a proof of concept to show that a state estimation oracle is not required to maintain safety (as is assumed by previous works).}

3. From my understanding, the introduced method can be only applied to visual feedback. If so, methods with regular CBFs and state estimation is more general and can deal with various sensors.

\textbf{Visual feedback is widely used by robots to explore novel, complex environments, particularly in GPS-denied environments, so our method is in fact greatly meaningful to practical applications in robotics.}

4. The task in the simulation is not difficult. The baseline method fails with a single integrator example. Is it the right method to compare? Is it the state-of-the-art for the considered problem?

\textbf{Sure, it is the right as well as the state-of-the-art method. As in some occasions the density map can be roughly constructed, which might cause danger like collision (as shown in contrast experiments for NeRF-Navigation), this is an instinct potential drawback of using density maps to judge the safety of the system. In this way, almost all the methods based on density maps can lead to failure including collision. However, our method directly utilizes the observed depth data to ensure the security, so it can avoid this flaw at ease.}

5. Is the RGB information used in the method or just the depth information? The author should make this clear and explain what is the visual feedback here.

\textbf{We do not use RGB data to help judge the safety of the intended action. We will lay emphasis on this point in the article.}
